The Darkside-20k Data Acquisition System

DarkSide-20k is a WIMP search experiment using liquid argon as a target, designed to perform a background-free search for dark matter with unprecedented sensitivity, and is currently under construction at INFN Laboratori Nazionali del Gran Sasso, Italy. The detector comprises a dual-phase Time Projection Chamber complemented with external veto systems and is equipped with a total of 2720 SiPM-based readout channels. This work presents the DAQ system designed for DarkSide-20k. The system is capable of continuous, triggerless digitisation of the waveforms with high single-photoelectron detection efficiency and online processing, ensuring data reduction for long-term storage. The DarkSide-20k DAQ system employs commercial CAEN VX2745 digitisers with custom FPGA firmware implementation. Timing and synchronisation across all 48 digitisers are provided by custom Global and Crate Data Manager boards distributing a phase-aligned clock derived from a disciplined rubidium standard. Waveform segments are processed in real time by Front End Processor machines. Data are organised into collections containing whole detector information and distributed across a farm of Time Slice Processors for event reconstruction, classification, and further reduction before storage and offline analysis. A full "Quadrant" of the system, corresponding to one quarter of the final DAQ, has been assembled and validated at TRIUMF laboratory in Canada. The Quadrant has been stress-tested with simultaneous pulses and demonstrated sustained digitizer readout exceeding expected physics rates and stable long-term performance.

==> DS20k-authors-march-17-2026-DAQ-PAPER.tex <==
% ===== Authors (alphabetical by Last, First, Middle) =====
\author[1]{Fabio Acerbi}
\author[2]{Pushparaj Adhikari}
\author[3,4]{Paolo Agnes}
\author[5]{Iftikhar Ahmad}
\author[6,7]{Sebastiano Albergo}
\author[8]{Ivone F.M. Albuquerque}
\author[9]{Thomas Alexander}
\author[10]{Andrew Knight Alton}
\author[11]{Pierre-Andr\'e Amaudruz}
\author[6,7]{Gioacchino Alex Anastasi}
\author[4,3]{Michele Angiolilli}
\author[12]{Elena Aprile}
\author[13]{David J. Auty}
\author[3]{Maximo Ave Pernas}
\author[14]{Oscar Azzolini}
\author[9]{Henning Olling Back}
\author[15]{Zoe Balmforth}
\author[16]{Ana Isabel Barrado Olmedo}
\author[17]{Pierre Barrillon}
\author[18,19]{Giovanni Batignani}
\author[20]{Swadheen Bharat}
\author[21]{Pritindra Bhowmick}
\author[22,23]{Sofia Blua}
\author[24]{Valerio Bocci}
\author[25]{Walter Bonivento}
\author[26,27]{Bianca Bottino}
\author[2]{Mark G. Boulay}
\author[21]{Titanilla Braun}
\author[28]{Andrzej Buchowicz}
\author[29,30]{Severino Bussino}
\author[17]{Jos\'e Busto}
\author[25]{Matteo Cadeddu}
\author[25]{Mariano Cadoni}
\author[31,32]{Roberta Calabrese}
\author[33]{Vincenzo Camillo}
\author[27]{Alessio Caminata}
\author[11]{Andrea Capra} %% added author
\author[31]{Nicola Canci}
\author[25]{Mauro Caravati}
\author[16]{Miguel C\'ardenas-Montes}
\author[25]{Nicola Cargioli}
\author[4]{Marco Carlini}
\author[25]{Paolo Castello}
\author[4]{Paolo Cavalcante}
\author[20]{Susana Cebrian}
\author[5]{Sarthak Choudhary}
\author[34,35]{Luisa Cifarelli}
\author[17]{Yann Coadou}
\author[20]{Iv\'an Coarasa}
\author[25]{Valentina Cocco}
\author[16]{Estefania Conde Vilda}
\author[4]{Lucia Consiglio}
\author[33]{Harrison Coombes}
\author[5]{Andr\'e Filipe Ventura Cortez}
\author[8]{Barbara S. Costa}
\author[36]{Milena Czubak}
\author[37,38]{Saverio D'Auria}
\author[22]{Manuel Dionisio Da Rocha Rolo}
\author[39]{Alexander Dainty}
\author[27]{Giovanni Darbo}
\author[27]{Stefano Davini}
\author[31]{Riccardo de Asmundis}
\author[40,24]{Sandro De Cecco}
\author[6,7]{Marzio De Napoli}
\author[22]{Giulio Dellacasa}
\author[27,26]{Lea Di Noto}
\author[41]{Philippe Di Stefano}
\author[16]{Daniel D\'iaz Mairena}
\author[40,24]{Carlo Dionisi}
\author[25]{Francesca Dordei}
\author[42]{Aaron Elersich}
\author[43]{Emma Ellingwood}
\author[42]{Tyler Erjavec}
\author[21]{Niamh Fearon}
\author[16]{Marta Fernandez Diaz}
\author[25,44]{Luca Ferro}
\author[1]{Andrea Ficorella}
\author[32,31]{Giuliana Fiorillo}
\author[42]{Dylon Fleming}
\author[21]{Paolo Franchini}
\author[45]{Davide Franco}
\author[46]{Heriques Frandini Gatti}
\author[25]{Federico Gabriele}
\author[4]{Devidutta Gahan}
\author[47]{Cristiano Galbiati}
\author[28]{Grzegorz Gali\'nski}
\author[47]{Giacomo Gallina}
\author[35,48]{Marco Garbini}
\author[16]{Pablo Garcia Abia}
\author[49]{Andrzej Gawdzik}
\author[50]{Graham Kurt Giovanetti}
\author[1]{Alberto Gola}
\author[51]{Luca Grandi}
\author[31]{Gianfrancesco Grauso}
\author[4]{Giovanni Grilli di Cortona}
\author[16]{Juli\'an Guerrero C\'anovas}
\author[52,53]{Marisa Gulino}
\author[5]{Samuel Belayneh Habtemariam}
\author[9]{Brianne Rae Hackett}
\author[13]{Aksel Hallin}
\author[36]{Malgorzata Haranczyk}
\author[45]{Timoth\'ee Hessel}
\author[3]{Celin Hidalgo}
\author[39]{James Hollingham}
\author[54]{Sosuke Horikawa}
\author[13]{Jie Hu}
\author[17]{Fabrice Hubaut}
\author[55]{Daniel Huff}
\author[41]{Th\'eo Hugues}
\author[47]{Andrea Ianni}
\author[24]{Valerio Ippolito}
\author[47]{Ako Jamil}
\author[56,57]{Chris Jillings}
\author[33]{Rijeesh Keloth}
\author[8]{N\'ikolas Kemmerich}
\author[39]{Ashlea Kemp}
\author[4,58]{Kaori Kondo}
\author[59]{George Korga}
\author[43]{Lucy Kotsiopoulou}
\author[59]{Seraphim Koulosousas}
\author[3]{Pablo Kunz\'e}
\author[18]{Michael Kuss}
\author[5]{Marcin Ku\'zniak}
\author[5]{Maciej Kuzwa}
\author[60,31]{Marco La Commara}
\author[41]{Michela Lai}
\author[17]{Emmanuel Le Guirriec}
\author[21]{Elizabeth Leason}
\author[4,58]{Alfiero Leoni}
\author[9]{Lance Lidey}
\author[39]{John D Lipp}
\author[25]{Marcello Lissia}
\author[42]{Ludovico Luzzi}
\author[50]{Oliver Macfadyen}
\author[45]{Janna Machts}
\author[56,57]{Szymon Manecki}
\author[15]{Ioannis Manthos}
\author[4]{Andrea Marasciulli}
\author[29,30]{Stefano Maria Mari}
\author[33]{Camillo Mariani}
\author[54]{Jelena Maricic}
\author[20]{Maria Martinez}
\author[32,31]{Giuseppe Matteucci}
\author[46]{Konstantinos Mavrokoridis}
\author[41]{Arthur B. McDonald}
\author[51]{Luo Meng}
\author[1]{Stefano Merzi}
\author[40]{Andrea Messina}
\author[54]{Radovan Milincic}
\author[49]{Graham Miller}
\author[27]{Saverio Minutoli}
\author[61]{Ankush Mitra}
\author[21]{Jocelyn Monroe}
\author[18]{Matteo Morrocchi}
\author[62]{Abdulrahman Morsy}
\author[12]{Michael Murra}
\author[25]{Carlo Muscas}
\author[27]{Paolo Musico}
\author[35]{Rosario Nania}
\author[63]{Marzio Nessi}
\author[5]{Grzegorz Nieradka}
\author[15]{Konstantinos Nikolopoulos}
\author[45]{Evangelia Nikoloudaki}
\author[64]{Jaroslaw Nowak}
\author[11]{Konstantin Olchanski}
\author[4,47]{Paolo Organtini}
\author[20]{Alfonso Ortiz de Sol\'orzano}
\author[41]{Anantha Padmanabhan}
\author[26,27]{Marco Pallavicini}
\author[52]{Luciano Pandola}
\author[42]{Emilija Pantic}
\author[18,19]{Eugenio Paoloni}
\author[13]{Danial Papi}
\author[13]{Byungju Park}
\author[28]{Grzegorz Pastuszak}
\author[1]{Giovanni Paternoster}
\author[25,44]{Riccardo Pavarani}
\author[65]{Alec Peck}
\author[25]{Paolo Attilio Pegoraro}
\author[36]{Krzysztof Pelczar}
\author[8]{Ramon Perez}
\author[16]{Vicente Pesudo}
\author[3]{Stefano Piacentini}
\author[52]{Noemi Pino}
\author[12]{Guillaume Plante}
\author[62]{Andrea Pietro Pocar}
\author[33]{Stephen Pordes}
\author[17]{Pascal Pralavorio}
\author[47]{Elettra Preosti}
\author[49]{Darren Price}
\author[21]{George Prior}
\author[17]{Manuel Pronesti}
\author[6,7]{Sebastiana Puglia}
\author[46]{Maria Cecilia Queiroga Bazetto}
\author[18]{Fabrizio Raffaelli}
\author[37]{Francesco Ragusa}
\author[61]{Yorck Ramachers}
\author[55]{Alejandro Ramirez}
\author[46]{Sudikshan Ravinthiran}
\author[25]{Marco Razeti}
\author[55]{Andrew Lee Renshaw}
\author[65]{Aras Repond}
\author[24]{Marco Rescigno}
\author[38]{Silvia Resconi}
\author[11]{Fabrice Retiere}
\author[49]{Ash Ritchie-Yates}
\author[22]{Angelo Rivetti}
\author[46]{Adam Roberts}
\author[49]{Conner Roberts}
\author[5]{Diego Rodr\'iguez Rodas}
\author[66]{Giovanni Rogers}
\author[16]{Luciano Romero}
\author[26]{Matteo Rossi}
\author[32,31]{Dmitry Rudik}
\author[62]{James Runge}
\author[24]{Maria Adriana Sabia}
\author[3]{Camilla Salerno}
\author[24]{Paolo Salomone}
\author[52]{Simone Sanfilippo}
\author[21]{Daria Santone}
\author[16]{Roberto Santorelli}
\author[8]{Edivaldo M. Santos}
\author[39]{Isobel Sargeant}
\author[20]{Mar\'ia Luisa Sarsa}
\author[67]{Claudio Savarese}
\author[35]{Eugenio Scapparone}
\author[41]{Fred Schuckman}
\author[20]{Carmen Seoane}
\author[25,44]{Michela Sestu}
\author[65]{Veronika Shalamova}
\author[55]{Sanjay Sharma Poudel}
\author[68]{Marino Simeone}
\author[41]{Peter Skensved}
\author[65]{Taisiia Smirnova}
\author[11]{Ben Smith}
\author[39]{Robert Smith} % author added
\author[9]{Franco Spadoni}
\author[61]{Martin Spangenberg}
\author[25]{Arianna Steri}
\author[4,58]{Vincenzo Stornelli}
\author[18]{Simone Stracka}
\author[47]{Allan Sung}
\author[5]{Clea Sunny}
\author[32,31]{Yury Suvorov}
\author[43]{Andrzej M Szelc}
\author[3]{Oscar Taborda}
\author[21]{Benjamin Tam}
\author[4]{Roberto Tartaglia}
\author[46]{Alan Taylor}
\author[46]{Jonathan Taylor}
\author[27]{Gemma Testera}
\author[54]{Kevin Thieme}
\author[59]{Angus Thompson}
\author[55]{Sebastian Torres-Lara}
\author[6,7]{Alessia Tricomi}
\author[25,44]{Sara Tullio}
\author[21]{Marie Van Uffelen}
\author[8]{Pedro Ventura}
\author[16]{Guillermo Vera D\'iaz}
\author[2]{Simon Viel}
\author[33]{Bruce Vogelaar}
\author[46]{Joost Vossebeld}
\author[2]{Bansari Vyas}
\author[5]{Masayuki Wada}
\author[3]{Marek Bohdan Walczak}
\author[69,70]{Yi Wang}
\author[65]{Shawn Westerdale}
\author[71]{Laurie Williams}
\author[36]{Marcin Marian Wojcik}
\author[72]{Mariusz Wojcik}
\author[69,70]{Changgen Yang}
\author[69,70]{Jilong Yin}
\author[5]{Azam Zabihi}
\author[7,6]{Paul Zakhary}
\author[38]{Andrea Zani}
\author[49]{Haoxiang Zhan}
\author[69,70]{Yongpeng Zhang}
\author[34,35]{Antonino Zichichi$^\dagger$ }
\author[36]{Grzegorz Zuzel}

% ===== Affiliations (in increasing order of first appearance in sorted authors) =====
\affiliation[1]{Fondazione Bruno Kessler, Povo, 38123, Italy}
\affiliation[2]{Department of Physics, Carleton University, Ottawa, ON K1S 5B6, Canada}
\affiliation[3]{Gran Sasso Science Institute, L'Aquila, 67100, Italy}
\affiliation[4]{INFN Laboratori Nazionali del Gran Sasso, Assergi (AQ), 67100, Italy}
\affiliation[5]{AstroCeNT, Nicolaus Copernicus Astronomical Center of the Polish Academy of Sciences, Warsaw, 00-614, Poland}
\affiliation[6]{INFN Catania, Catania, 95121, Italy}
\affiliation[7]{Universit\`a of Catania, Catania, 95124, Italy}
\affiliation[8]{Instituto de F\'isica, Universidade de S\~ao Paulo, S\~ao Paulo, 05508-090, Brazil}
\affiliation[9]{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\affiliation[10]{Physics Department, Augustana University, Sioux Falls, SD 57197, USA}
\affiliation[11]{TRIUMF, 4004 Wesbrook Mall, Vancouver, BC V6T 2A3, Canada}
\affiliation[12]{Physics Department, Columbia University, New York, NY 10027, USA}
\affiliation[13]{Department of Physics, University of Alberta, Edmonton, AB T6G 2R3, Canada}
\affiliation[14]{INFN Laboratori Nazionali di Legnaro, Legnaro (Padova), 35020, Italy}
\affiliation[15]{Institute for Experimental Physics, University of Hamburg, 22761, Germany}
\affiliation[16]{CIEMAT, Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, Madrid, 28040, Spain}
\affiliation[17]{Centre de Physique des Particules de Marseille, Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}
\affiliation[18]{INFN Pisa, Pisa, 56127, Italy}
\affiliation[19]{Physics Department, Universit\`a degli Studi di Pisa, Pisa, 56127, Italy}
\affiliation[20]{Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias, Universidad de Zaragoza, Zaragoza, 50009, Spain}
\affiliation[21]{Department of Physics, University of Oxford, Oxford, OX1 3RH, UK}
\affiliation[22]{INFN Torino, Torino, 10125, Italy}
\affiliation[23]{Department of Electronics and Communications, Politecnico di Torino, Torino, 10129, Italy}
\affiliation[24]{INFN Sezione di Roma, Roma, 00185, Italy}
\affiliation[25]{INFN Cagliari, Cagliari, 09042, Italy}
\affiliation[26]{Physics Department, Universit\`a degli Studi di Genova, Genova, 16146, Italy}
\affiliation[27]{INFN Genova, Genova, 16146, Italy}
\affiliation[28]{Warsaw University of Technology, Warsaw, 00-661, Poland}
\affiliation[29]{INFN Roma Tre, Roma, 00146, Italy}
\affiliation[30]{Mathematics and Physics Department, Universit\`a degli Studi Roma Tre, Roma, 00146, Italy}
\affiliation[31]{INFN Napoli, Napoli, 80126, Italy}
\affiliation[32]{Physics Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli, 80126, Italy}
\affiliation[33]{Virginia Tech, Blacksburg, VA 24061, USA}
\affiliation[34]{Department of Physics and Astronomy, Universit\`a degli Studi di Bologna, Bologna, 40126, Italy}
\affiliation[35]{INFN Bologna, Bologna, 40126, Italy}
\affiliation[36]{M. Smoluchowski Institute of Physics, Jagiellonian University, Krakow, 30-348, Poland}
\affiliation[37]{Physics Department, Universit\`a degli Studi di Milano, Milano, 20133, Italy}
\affiliation[38]{INFN Milano, Milano, 20133, Italy}
\affiliation[39]{Science \& Technology Facilities Council (STFC), Rutherford Appleton Laboratory, Technology, Harwell Oxford, Didcot, OX11 0QX, UK}
\affiliation[40]{Physics Department, Sapienza Universit\`a di Roma, Roma, 00185, Italy}
\affiliation[41]{Department of Physics, Engineering Physics and Astronomy, Queen's University, Kingston, ON K7L 3N6, Canada}
\affiliation[42]{Department of Physics, University of California Davis, Davis, CA 95616, USA}
\affiliation[43]{School of Physics and Astronomy, University of Edinburgh, Edinburgh, EH9 3FD, UK}
\affiliation[44]{Physics Department, Universit\`a degli Studi di Cagliari, Cagliari, 09042, Italy}
\affiliation[45]{APC, Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, Paris, F-75013, France}
\affiliation[46]{Department of Physics, University of Liverpool, The Oliver Lodge Laboratory, Liverpool, L69 7ZE, UK}
\affiliation[47]{Physics Department, Princeton University, Princeton, NJ 08544, USA}
\affiliation[48]{Museo Storico della Fisica e Centro Studi e Ricerche Enrico Fermi, Roma, 00184, Italy}
\affiliation[49]{Department of Physics and Astronomy, The University of Manchester, Manchester, M13 9PL, UK}
\affiliation[50]{Williams College, Department of Physics and Astronomy, Williamstown, MA 01267, USA}
\affiliation[51]{Department of Physics and Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\affiliation[52]{INFN Laboratori Nazionali del Sud, Catania, 95123, Italy}
\affiliation[53]{Engineering and Architecture Department, Universit\`a di Enna Kore, Enna, 94100, Italy}
\affiliation[54]{Department of Physics and Astronomy, University of Hawai'i, Honolulu, HI 96822, USA}
\affiliation[55]{Department of Physics, University of Houston, Houston, TX 77204, USA}
\affiliation[56]{Department of Physics and Astronomy, Laurentian University, Sudbury, ON P3E 2C6, Canada}
\affiliation[57]{SNOLAB, Lively, ON P3Y 1N2, Canada}
\affiliation[58]{Universit\`a degli Studi dell'Aquila, L'Aquila, 67100, Italy}
\affiliation[59]{Department of Physics, Royal Holloway University of London, Egham, TW20 0EX, UK}
\affiliation[60]{Pharmacy Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli, 80131, Italy}
\affiliation[61]{University of Warwick, Department of Physics, Coventry, CV47AL, UK}
\affiliation[62]{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\affiliation[63]{Istituto Nazionale di Fisica Nucleare, Roma, 00186, Italia}
\affiliation[64]{Physics Department, Lancaster University, Lancaster, LA1 4YB, UK}
\affiliation[65]{Department of Physics and Astronomy, University of California Riverside, Riverside, CA 92507, USA}
\affiliation[66]{School of Physics and Astronomy, University of Birmingham, Edgbaston, Birmingham, B15 2TT, UK}
\affiliation[67]{Center for Experimental Nuclear Physics and Astrophysics, and Department of Physics, University of Washington, Seattle, WA 98195, USA, Seattle, WA 98195, USA}
\affiliation[68]{Chemical, Materials, and Industrial Production Engineering Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli, 80126, Italy}
\affiliation[69]{Institute of High Energy Physics, Beijing, 100049, China}
\affiliation[70]{University of Chinese Academy of Sciences, Beijing, 100049, China}
\affiliation[71]{Department of Physics and Engineering, Fort Lewis College, Durango, CO 81301, USA}
\affiliation[72]{Institute of Applied Radiation Chemistry, Lodz University of Technology, Lodz, 93-590, Poland}
\affiliation[\dagger]{Deceased}


==> acknowledgements-DS20k-mar-2026-v2.tex <==
This work was supported by the U.S. National Science Foundation
(NSF) through Grants No. PHY-0919363, PHY-1004054, PHY-1004072,
PHY-1242585, PHY-1314483, PHY-1314507, PHY-1622337, PHY-1812482,
PHY-1812547, PHY-2310091, PHY-2310046, associated collaborative
grants No. PHY-1211308, PHY-1314501, PHY-1455351 and PHY-1606912, as
well as Major Research Instrumentation Grant No. MRI-1429544.
Additional support was provided by the Pacific Northwest National
Laboratory, operated by Battelle for the U.S. Department of Energy
under Contract No. DE-AC05-76RL01830.

Support was provided by the Istituto Nazionale di Fisica Nucleare
(INFN), through grants from the Italian Ministero dell’Istruzione,
Università e Ricerca, including Progetto Premiale 2013 and
Commissione Scientifica Nazionale II, as well as by the PRIN2020
project of the Italian Ministry of Research (MUR) (Grant No. PRIN
20208XN9TZ).

This work was supported by Canada Foundation for Innovation (CFI), the Natural Sciences and Engineering
Research Council of Canada, SNOLAB, and the Arthur B. McDonald
Canadian Astroparticle Physics Research Institute.
Support was received from the French government from LabEx
UnivEarthS (ANR-10-LABX-0023 and ANR-18-IDEX-0001). Additional
support was received from the IN2P3-COPIN consortium (Grant No.
20-152).

This work was supported by the Chinese Academy of Sciences
(113111KYSB20210030) and the National Natural Science Foundation of
China (12020101004).
Support was provided by the São Paulo Research Foundation (FAPESP)
under Grant No. 2021/11489-7 and by the National Council for
Scientific and Technological Development (CNPq).
Support is acknowledged from the Deutsche Forschungsgemeinschaft
(DFG, German Research Foundation) under Germany’s Excellence
Strategy — EXC 2121: Quantum Universe — 390833306.

The authors acknowledge support from the Spanish Ministry of Science
and Innovation (MICINN) through Grants PID2022-138357NB-C22 and
PID2022-138357NB-C21 and the Atracción de Talento Grant 2018-T2/
TIC-10494.

This work was supported by the Polish National Science Centre (NCN)
through Grants No. UMO-2022/47/B/ST2/02015 and UMO-2023/51/B/
ST2/02099, by the Polish Ministry of Science and Higher Education
(MNiSW, Grant No. 6811/IA/SP/2018).
This work was supported by the FNP IRA programmes: AstroCeNT
(MAB/2018/7), funded from the ERDF, and Astrocent
(FENG.02.01-IP.05-A015/25) co-financed by the European Union under
FENG 2021–2027; and Teaming for Excellence grant Astrocent Plus
(101137080)
funded by the European Union with complementary national funding from
the MNiSW (MNiSW/2025/DIR/811).

This project received funding from the European Union’s Horizon 2020
research and innovation programme under Grant Agreement No. 952480
(DarkWave).

Support was provided by the Science and Technology Facilities
Council, part of United Kingdom Research and Innovation, and by The
Royal Society.
